Generalized Additive Models for Pair-Copula Constructions

Pair-copula constructions are flexible dependence models that use bivariate copulas as building blocks. In this paper, we use generalized additive models to extend them by allowing covariates effects. Borrowing ideas from a traditionally univariate context, we let each pair-copula parameter depend directly on the covariates in a parametric, semiparametric or nonparametric way. We propose a sequential estimation method that we study by simulation, and apply it to investigate the time-varying dependence structure between the intraday returns on four major foreign exchange rates. An R package, a script reproducing the results in this article, and additional simulation results are provided as supplementary material.

==> tex/pccs.tex <==
\section{Some background on pair-copula constructions}

\label{sec:pcc}

This section gives a brief introduction to pair-copula constructions. For a more extensive treatment, we refer to \citet{aasczadofrigessibakken2009} and \cite{czado2010}. By the famous theorem of \citet{Sklar59}, any multivariate distribution function $F$ can be represented by its marginal distributions $F_1, \dots, F_d$ and a \emph{copula} $C$:
\begin{align*}
    F(x_1, \dots, x_d) = C\bigl(F_1(x_1), \dots, F_d(x_d)\bigr)
\end{align*}The copula $C$ describes the dependence structure of the random vector $\bm X$ and is the joint distribution of the random vector $\bm U = (U_1, \dots, U_d) = \bigl(F_1(X_1), \dots, F_d(X_d)\bigr)$. If $F$ admits a density, we can differentiate the above equation to get
\begin{align*}
    f(x_1, \dots, x_d) = c\bigl(F_1(x_1), \dots, F_d(x_d)\bigr) \times \prod_{k=1}^d f_k(x_k),
\end{align*}
where $c, f_1, \dots, f_d$ are the probability density functions corresponding to $C, F_1, \dots, F_d$ respectively. 

A pair-copula construction is a graphical model for the dependence underlying a $d$-variate random vector $\bm X = (X_1, \dots, X_d) \sim F$. Following the seminal work of \citet{Joe97} and \citet{Bedford01, Bedford02}, any copula density $c$ can be decomposed into a product of $d(d-1)/2$ bivariate (conditional) copula densities. The decomposition is not unique, but all possible decompositions can be organized as graphical structure, called \emph{regular vine (R-vine)} - a sequence of trees $T_m = (V_m, E_m), m = 1, \dots, d-1$ satisfying the following conditions:
	\begin{enumerate}
		\item $T_1$ is a tree with nodes $V_1=\{1, \dots, d\}$ and edges $E_1$.
		\item For $m\ge 2$, $T_m$ is a tree with nodes $V_m=E_{m-1}$ and edges $E_m$.
		\item (\emph{Proximity condition}) Whenever two nodes in $T_{m+1}$ are joined by an edge, the corresponding edges in $T_m$ must share a common node.
	\end{enumerate}   
The corresponding tree sequence is also called the \emph{structure} of the PCC. A PCC identifies each edge $e$ of the trees with a bivariate copula $c_{j_e, k_e ; D_e}$ (a so-called \emph{pair-copula}). The joint density of the PCC can then be written as the product of all pair-copula densities:
\begin{align}
c(\bm u) = \prod_{m=1}^{d-1} \prod_{e \in E_m} c_{j_e, k_e; D_e} \bigl(C_{j_e|D_e}(u_{j_e}|\bm u_{D_e}), C_{k_e|D_e}(u_{k_e}|\bm u_{D_e}) ; \, \bm u_{D_e} \bigr), \label{sec:gampcc:density_nonsimplified_eq}
\end{align}
where $\bm u_{D_e}:=(u_\ell)_{\ell \in D_e}$ is a subvector of $\bm u =(u_1, \dots, u_d) \in [0,1]^d$ and $C_{j_e|D_e}$ is the conditional distribution of $U_{j_e} | \bm U_{D_e} = \bm u_{D_e}$. The set $D_e$ is called \emph{conditioning set} and the indices $j_e, k_e$ form the \emph{conditioned set}. Put differently, the pair-copula density $c_{j_e, k_e; D_e}$ describes the dependence between the two variables $U_{j_e}$ and $U_{k_e}$, conditional on $\bm U_{D_e} = u_{D_e}$.

\begin{Example}   \label{sec:gampcc:vine_ex}
	The density of a PCC corresponding to the tree sequence in \autoref{sec:gampcc:RVine_fig} is
	\begin{align*}
	c(u_1, \dots, u_5) &= c_{1,2}(u_1, u_2) \times c_{1,3}(u_1,u_3) \times c_{3,4}(u_3,u_4) \times c_{3,5}(u_3,u_5)\\
	& \phantom{=} \times c_{2,3;1}(u_{2|1}, u_{3|1}; u_1) \times c_{1,4;3}(u_{1|3}, u_{4|3}; u_3) \times c_{1,5;3}(u_{1|3}, u_{5|3}; u_3) \\
	& \phantom{=} \times c_{2,4;1,3}(u_{2|1,3}, u_{4|1,3}; \bm u_{\{1,3\}}) \times c_{4,5;1,3}(u_{4|1,3}, u_{5|1,3}; \bm u_{\{1,3\}}) \\
	& \phantom{=} \times c_{2,5;1,3,4}(u_{2|1,3,4}, u_{5|1,3,4}; \bm u_{\{1,3,4\}}),
	\end{align*}
	where we used the abbreviation $u_{j_e|D_e} := C_{j_e|D_e}(u_{j_e}|\bm u_{D_e})$.
\end{Example}
\begin{figure}
	%\includegraphics[width=\textwidth]{images/Rvine.pdf}
	\input{tikz/rvineex}
	\caption{Example of a regular vine tree sequence.}
	\label{sec:gampcc:RVine_fig}
\end{figure}
%\autoref{sec:gampcc:RVine_fig} shows an example of an R-vine tree sequence for $d=5$.

==> tikz/nonsimpex.tex <==
\begin{minipage}[t]{.32\linewidth}
     \centering
\begin{tikzpicture}[node distance=2cm,>=latex']
\node [nn1] (U1) {$1$};
\node [nn1, above left =1cm of U1] (U2) {$2$};
\draw [ee1] (U1) --  node {$1,2$} (U2) ;
\node [nn1, above right = 1cm of U1] (U3) {$3$};
\draw [ee1] (U1) --  node {$1,3$} (U3) ;
\node [nn1, below left =1cm of U1] (U4) {$4$};
\draw [ee1] (U1) --  node {$1,4$} (U4) ;
\end{tikzpicture}
\label{fig:nonsimpex1}
\vspace*{0.5cm}
\subcaption{$T_1$}
\end{minipage} 
\begin{minipage}[t]{.32\linewidth}
     \centering
\begin{tikzpicture}[node distance=2cm,>=latex']
\node [nn1] (U1) {$1,4$};
\node [nn1, below left = 2.5cm of U1] (U2) {$1,2$};
\draw [ee1] (U1) --  node {$2,4;1$} (U2) ;
\node [nn1, below right = 2.5cm of U1] (U3) {$1,3$};
\draw [ee1] (U1) --  node {$3,4;1$} (U3) ;
\end{tikzpicture}
\label{fig:nonsimpex2}
\subcaption{$T_2$}
\end{minipage} 
\begin{minipage}[t]{.32\linewidth}
     \centering
\begin{tikzpicture}[node distance=2cm,>=latex']
\node [nn1] (U1) {$2,4;1$};
\node [nn1, below =1.6cm of U1] (U2) {$3,4;1$};
\draw [ee1] (U1) --  node {$2,3;1,4$} (U2) ;
\end{tikzpicture}
\label{fig:nonsimpex3}
\vspace*{0.5cm}
\subcaption{$T_3$}
\end{minipage}

==> tikz/uranium_trees.tex <==
\tikzstyle{VineNode} = [ellipse, fill = white, draw = black, text = black, align = center]
\tikzstyle{DummyNode}  = [draw = none, fill = none, text = white] % Weisser Node ohne Text zum besseren Ausrichten
\tikzstyle{TreeLabels} = [draw = none, fill = none, text = black] % T_1, T_2, etc.
\newcommand{\labelsize}{\footnotesize} % Groesse edge labels
\newcommand{\yshiftLabel}{-0.3cm}  % Abstand der Labels zu Edges reduzieren (ausprobieren)
\newcommand{\yshiftNodes}{-0.75cm} % Abstand der Zeilen der Graphik (ausprobieren)
\newcommand{\xshiftTree}{0.5cm}    % Abstand der Baume (Mittelpunkt der Nodes) (ausprobieren)
\newcommand{\rotateLabels}{-57}    % Drehung der Labels an Edges (wenn yshift weggelassen wird, dann z.B bei 1,3 -45 Grad)
	\centering
	\begin{tikzpicture}	[every node/.style = VineNode, node distance =1.6cm, minimum width = 1cm, minimum height = 1cm] % node distance = Skalierung Edges (ausprobieren)
	%%% Tree 1 nodes
	\node (Co){3}
	node  (Sc) [right of = Co, xshift = 0.7cm] {6}
    node  (Ti) [right of = Sc, xshift = 0.7cm] {7}
    node  (Cs) [right of = Ti, xshift = 0.7cm] {5}
    node  (K) [below right of = Cs, xshift = 1.0cm] {4}
    node  (U) [above right of = Cs, xshift = 1.0cm] {1}
    node  (Li)  [above right of = U, xshift = 1.0cm] {2}
    %%% Tree 2 nodes
	node (Sc_Co) [below of = Co, yshift = -1.8cm] {$3,6$}
    node (Ti_Sc) [right of = Sc_Co, xshift = 1.5cm] {$6,7$}
    node (Ti_Cs) [right of = Ti_Sc, xshift = 1.5cm] {$7,5$}
    node (Cs_U)  [right of = Ti_Cs, xshift = 1.5cm] {$5,1$}
    node (Cs_K)  [below right of = Cs_U, xshift = 1.8cm]  {$5,4$}
    node (U_Li)  [above right of = Cs_U, xshift = 1.8cm]  {$1,2$}
    %%% Tree 3 nodes
    node (Ti_Co-Sc) [below of = Sc_Co, yshift = -2.3cm] {$3,7;6$}
    node (Sc_Cs-Ti) [right of = Ti_Co-Sc, xshift = 1.9cm] {$6,5;7$}
    node (Ti_U-Cs) [right of = Sc_Cs-Ti, xshift = 1.9cm] {$7,1;5$}
    node (Cs_Li-U) [above right = 1cm  of  Ti_U-Cs, xshift = 1.9cm] {$5,2;1$}
    node (U_K-Cs) [below right = 1cm  of  Ti_U-Cs, xshift = 1.9cm] {$1,4;5$}
    %%% Tree 4 nodes
%     node (Cs_Co-Ti_Sc) [below of = Ti_Cs, yshift = -2cm, xshift = -1.2cm] {Cs, Co;Ti, Sc}
%     node (Sc_U-Ti_Cs) [below of = Cs_Co-Ti_Sc] {Sc, U;Ti, Cs}
%     node (Ti_K-U_Cs) [below left = 0.7cm of Sc_U-Ti_Cs] {Ti, K;U, Cs}
%     node (Ti_Li-U_Cs) [below right = 0.7cm of Sc_U-Ti_Cs] {Ti, Li;U, Cs}
%     %%% Tree 5 nodes
%     node (Sc_Li-Ti_Cs_U) [right of = Cs_Co-Ti_Sc, xshift = 3cm] {Sc, Li;Ti,Cs,U}
	;
    %%% Tree 1 edge
    \draw[dotted] (Co) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = 0, above, yshift = \yshiftLabel] {$3,6$} (Sc); 
    \draw[dotted] (Sc) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = 0, above, yshift = \yshiftLabel] {$6,7$} (Ti); 
    \draw[dotted] (Ti) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = 0, above, yshift = \yshiftLabel] {$7,5$} (Cs);     
    \draw[dotted] (Cs) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = -30, above, yshift = \yshiftLabel] {$5,4$} (K);     
    \draw[dotted] (Cs) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = 30, above, yshift = \yshiftLabel] {$5,1$} (U); 
    \draw[dotted] (U) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = 30, above, yshift = \yshiftLabel] {$1,2$} (Li); 


    %%% Tree 2 edges  
	\draw (Sc_Co) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = 0, above, yshift = \yshiftLabel] {$3,7;6$} (Ti_Sc);   
	\draw (Ti_Sc) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = 0, above, yshift = \yshiftLabel] {$6,5;7$} (Ti_Cs);
	\draw[dotted] (Ti_Cs) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = 0, above, yshift = \yshiftLabel] {$7,1;5$} (Cs_U);  
	\draw[dotted] (Cs_U) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = 22, above, yshift = \yshiftLabel] {$5,2;1$} (U_Li);
	\draw[dotted] (Cs_U) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = -22, above, yshift = \yshiftLabel] {$1,4;5$} (Cs_K);
     %%% Tree 3 edges  
	\draw (Ti_Co-Sc) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = 0, above, yshift = \yshiftLabel] {$3,5;6,7$} (Sc_Cs-Ti);    
	\draw[dotted] (Sc_Cs-Ti) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = 0, above, yshift = \yshiftLabel] {$6,1;5,7$} (Ti_U-Cs); 	
	\draw[dotted] (Ti_U-Cs) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = -19, above, yshift = \yshiftLabel] {$7,4;1,5$} (U_K-Cs);     
	\draw[dotted] (Ti_U-Cs) to node[draw=none, fill = none, font = \labelsize, above, 
	                    rotate = 19, above, yshift = \yshiftLabel] {$7,2;1,5$} (Cs_Li-U);     
    \end{tikzpicture}
